Automated Importance Sampling via Optimal Control for Stochastic Reaction Networks: A Markovian Projection-based Approach

We propose a novel alternative approach to our previous work (Ben Hammouda et al., 2023) to improve the efficiency of Monte Carlo (MC) estimators for rare event probabilities for stochastic reaction networks (SRNs). In the same spirit of (Ben Hammouda et al., 2023), an efficient path-dependent measure change is derived based on a connection between determining optimal importance sampling (IS) parameters within a class of probability measures and a stochastic optimal control formulation, corresponding to solving a variance minimization problem. In this work, we propose a novel approach to address the encountered curse of dimensionality by mapping the problem to a significantly lower-dimensional space via a Markovian projection (MP) idea. The output of this model reduction technique is a low-dimensional SRN (potentially even one dimensional) that preserves the marginal distribution of the original high-dimensional SRN system. The dynamics of the projected process are obtained by solving a related optimization problem via a discrete $L^2$ regression. By solving the resulting projected Hamilton-Jacobi-Bellman (HJB) equations for the reduced-dimensional SRN, we obtain projected IS parameters, which are then mapped back to the original full-dimensional SRN system, resulting in an efficient IS-MC estimator for rare events probabilities of the full-dimensional SRN. Our analysis and numerical experiments reveal that the proposed MP-HJB-IS approach substantially reduces the MC estimator variance, resulting in a lower computational complexity in the rare event regime than standard MC estimators.

==> commands.tex <==
%%%%%%%%%%%%
% commands %
%%%%%%%%%%%%

%packages
\usepackage[leqno]{amsmath}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{enumerate}
\usepackage[round,longnamesfirst]{natbib}
\usepackage[bookmarksopen,pdfstartview=FitH]{hyperref}
\hypersetup{colorlinks,%
            citecolor=blue,%
            filecolor=blue,%
            linkcolor=blue,%
            urlcolor=blue}%
\usepackage{dsfont}
\usepackage{mathtools}
\usepackage[mathscr]{euscript}
\usepackage{nicefrac,booktabs,mathrsfs}
\usepackage{nth}
\usepackage[dvipsnames]{xcolor}
%\usepackage[color]{showkeys}
\definecolor{refkey}{gray}{0.5}
\definecolor{labelkey}{gray}{.7}
\usepackage[backgroundcolor=white,bordercolor=orange]{todonotes}
\usepackage{upgreek}
\usepackage[dvipsnames]{xcolor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amssymb}
\usepackage[mathscr]{euscript}
\usepackage{xspace}
\usepackage{epsfig,rotating}
\usepackage{graphicx}
\usepackage{subfig}
\input{xy}\xyoption{all}

\usepackage{lscape}
\usepackage{enumitem}
\usepackage{upgreek}
\usepackage{subfigure} 
\usepackage{epstopdf}

% \usepackage{txgreeks}
% \usepackage[T1]{fontenc}

\usepackage[left=1.10in,right=1.10in,top=1.40in,bottom=1.30in]{geometry}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


%%%%%%%%%%%%%

%Textstyles


%letters 
\renewcommand{\P}{\mathbb{P}} %probability
\newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\FF}{\mathbb{F}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cD}{\mathcal{D}}


%common math symbols
\def\half{\frac1{2}}
\newcommand{\ind}{\mathbbm1}

%other symbold, common names
\newcommand{\cadlag}{c{\'a}dl{\'a}g }
\newcommand{\Levy}{L{\'e}vy }


%common math notation
\newcommand{\cond}[1]{\left.#1\right\vert}%to get a vert with the right size

%brackets
\newcommand{\brac}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\Brac}[1]{\ensuremath{\big(#1\big)}}
\newcommand{\BRac}[1]{\ensuremath{\Big(#1\Big)}}
\newcommand{\BRAc}[1]{\ensuremath{\bigg(#1\bigg)}}
\newcommand{\BRAC}[1]{\ensuremath{\Bigg(#1\Bigg)}}

\newcommand{\brak}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\scal}[1]{\ensuremath{\left\langle#1\right\rangle}}
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}%doudle vert norm
\newcommand{\norm}[1]{\left\vert#1\right\vert}%single vert norm




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% ========================================================================== %%
%% ========================================================================== %%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{axiom}{Axiom}
\newtheorem{hypothesis}[theorem]{Hypothesis}  %[section]



\theoremstyle{definition*}
\newtheorem{example*}{Example}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{note}{Note}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem*{ackn}{Acknowledgements}
\newtheorem{assumption}{Assumption}
\newtheorem{approach}{Approach}
\newtheorem{critique}{Critique}
\newtheorem{question}{Question}
\newtheorem{aim}{Aim}
\newtheorem*{assucd}{Assumption ($\mathbb{CD}$)}
\newtheorem*{asa}{Assumption ($\mathbb{A}$)}
\newtheorem*{appS}{Approximation ($\mathbb{S}$)}
\newtheorem*{appBS}{Approximation ($\mathbb{BS}$)}
% \newtheorem*{asp}{Assumption ($\P$)}
% \newtheorem*{ass}{Assumption ($\mathbb{S}$)}
%% 


%% ========================================================================== %%
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\numberwithin{equation}{section}

\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\numberwithin{equation}{section}

\newcommand{\Law}{\ensuremath{\mathop{\mathrm{Law}}}}
\newcommand{\loc}{{\mathrm{loc}}}

\let\SETMINUS\setminus
\renewcommand{\setminus}{\backslash}

\def\stackrelboth#1#2#3{\mathrel{\mathop{#2}\limits^{#1}_{#3}}}

% \makeatletter
% \def\Ddots{\mathinner{\mkern1mu\raise\p@
% \vbox{\kern7\p@\hbox{.}}\mkern2mu
% \raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
% \makeatother
% 
% \newcommand\llambda{{\mathchoice
%      {\lambda\mkern-4.5mu{\raisebox{.4ex}{\scriptsize$\backslash$}}}
%      {\lambda\mkern-4.83mu{\raisebox{.4ex}{\scriptsize$\backslash$}}}
%      {\lambda\mkern-4.5mu{\raisebox{.2ex}
% {\footnotesize$\scriptscriptstyle\backslash$}}}
%      {\lambda\mkern-5.0mu{\raisebox{.2ex}
% {\tiny$\scriptscriptstyle\backslash$}}}}}

\newcommand{\prozess}[1][L]{{\ensuremath{#1=(#1_t)_{t\in[0,T]}}}\xspace}
\newcommand{\prazess}[1][L]{{\ensuremath{#1=(#1_t)_{t\ge0}}}\xspace}
\newcommand{\pt}[1][N]{\ensuremath{\P_{#1}}\xspace}
\newcommand{\tk}[1][N]{\ensuremath{T_{#1}}\xspace}
\newcommand{\dd}[1][]{\ensuremath{\ud{#1}}\xspace}


\newcommand{\bscal}[2]{\ensuremath{\big\langle #1, #2 \big\rangle}}

%\newcommand{\R}[1][\R]{\ensuremath{\R^{#1}}\xspace}
% \newcommand{\pt}[1][]{{\ensuremath{\P_{T^*_{#1}}}}\xspace}
% \newcommand{\ts}[1][]{\ensuremath{T^*_{#1}}\xspace}
%% ========================================================================== %%
%% ========================================================================== %%
\def\lev{L\'{e}vy\xspace}
\def\lk{L\'{e}vy--Khintchine\xspace}
\def\lib{LIBOR\xspace}
\def\mg{martingale\xspace}
\def\smmg{semimartingale\xspace}
\def\alm{affine LIBOR model\xspace}
\def\alms{affine LIBOR models\xspace}
\def\dalms{defaultable \alms}
\def\ap{affine process\xspace}
\def\aps{affine processes\xspace}

\def\half{\frac1{2}}

\def\F{\ensuremath{\mathcal{F}}}
\def\bD{\mathbf{D}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\R{\ensuremath{\mathbb{R}}}
\def\Rp{\mathbb{R}_{\geqslant0}}
\def\Rm{\mathbb{R}_{\leqslant 0}}
\def\C{\ensuremath{\mathbb{C}}}
\def\U{\ensuremath{\mathcal{U}}}
\def\I{\mathcal{I}}
\def\N{\mathbbN}

\def\P{\ensuremath{\mathbb P}} %{\ensuremath{\mathrm{I\kern-.2em P}}}
%\def\Q{\ensuremath{\mathrm{I\kern-.2em Q}}} % looks strange?
\def\Q{\mathbb{Q}}
\def\E{\ensuremath{\mathbb E}} %{\ensuremath{\mathrm{I\kern-.2em E}}}

\def\hP{\ensuremath{\widehat{\mathrm{I\kern-.2em P}}}}
\def\hE{\ensuremath{\widehat{\mathrm{I\kern-.2em E}}}}

\def\bP{\ensuremath{\overline{\mathrm{I\kern-.2em P}}}}
\def\bE{\ensuremath{\overline{\mathrm{I\kern-.2em E}}}}

\def\bphi{\overline{\phi}}
\def\bpsi{\overline{\psi}}

\def\ott{{0\leq t\leq T}}
\def\idd{{1\le i\le d}}

\def\icc{\mathpzc{i}}
\def\ecc{\mathbf{e}_\mathpzc{i}}

\def\uk{u_{k+1}}
\def\vk{v_{k+1}}

\def\e{\mathrm{e}}
\def\a{\mathrm{a}}
\def\b{\mathrm{b}}
\def\ud{\ensuremath{\mathrm{d}}}
\def\dt{\ud t}
\def\dr{\ud r}
\def\ds{\ud s}
\def\dx{\ud x}
\def\dy{\ud y}
\def\dv{\ud v}
\def\du{\ud u}
\def\dw{\ud w}
\def\dz{\ud z}
\def\dsdx{\ensuremath{(\ud s, \ud x)}}
\def\dtdx{\ensuremath{(\ud t, \ud x)}}

\def\rx{\mathrm{x}}

\def\1{\boldsymbol1}
\def\i{\mathrm{i}}
\def\wf{\widehat f}

\def\tc{\ensuremath{\mathpzc{T}}}
\def\afflm{\ensuremath{(X,\mathcal{X},T_N,u,v)}\xspace}

\def\lsnc{\ensuremath{\mathrm{LSNC-}\chi^2}}
\def\nc{\ensuremath{\mathrm{NC-}\chi^2}}


%% ========================================================================== %%
%% ========================================================================== %%

\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\ha}{{\mathbb{H}}}
\newcommand{\indik}{{\mathbf1}}
\newcommand{\ifdefault}[1]{\ensuremath{\mathbf1_{\{\tau \leq #1\}}}}
\newcommand{\ifnodefault}[1]{\ensuremath{\mathbf1_{\{\tau > #1\}}}}

\newcommand\bovermat[2]{%
    \makebox[0pt][l]{$\smash{\overbrace{\phantom{%
                    \begin{matrix}#2\end{matrix}}}^{#1}}$}#2}
\newcommand\bundermat[2]{%
    \makebox[0pt][l]{$\smash{\underbrace{\phantom{%
                    \begin{matrix}#2\end{matrix}}}_{#1}}$}#2}
\makeatletter



\newcommand{\robert}[1]{\todo[linecolor=blue!40!white,backgroundcolor=blue!20!white,size=\footnotesize]{Robert: #1}}

\def\red{\color{red}}
\def\blue{\color{magenta}}
\def\green{\color{OliveGreen}}

\newcommand{\rr}[1]{{\red #1}}
\newcommand{\rg}[1]{{\green #1}}
%% ========================================================================== %%
%% ========================================================================== %%
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%chiheb commands

\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\cf}{\emph{cf.}}
\newcommand{\prob}[1]{\mathrm{P}\left(#1\right)}
\newcommand{\expt}[1]{\mathrm{E}\left[#1\right]}
\newcommand{\expth}[1]{\hat{\mathrm{E}}\left[#1\right]}
\newcommand{\var}[1]{\mathrm{Var}\left[#1\right]}


\newcommand{\rset}{\mathbb{R}}
\newcommand{\nset}{\mathbb{N}}
\newcommand{\zset}{\mathbb{Z}}

\newcommand{\PERIOD}{.}
\newcommand{\COMMA}{,}
\newcommand{\BIGSPACE}{\,\,\,\,\,\,\,}



\newcommand{\Ordo}[1]{{\mathcal{O}}\left(#1\right)}
\newcommand{\ordo}[1]{{o}\left(#1\right)}


\newcommand{\latt}{\mbox{$\zset_+^d$}}


